Fair Allocation of Bandwidth At Edge Servers For Concurrent Hierarchical Federated Learning

This paper explores concurrent FL processes within a three-tier system, with edge servers between edge devices and FL servers. A challenge in this setup is the limited bandwidth from edge devices to edge servers. Thus, allocating the bandwidth efficiently and fairly to support simultaneous FL processes becomes crucial. We propose a game-theoretic approach to model the bandwidth allocation problem and develop distributed and centralized heuristic schemes to find an approximate Nash Equilibrium of the game. We proposed the approach mentioned above using centralized and entirely distributed assumptions. Through rigorous analysis and experimentation, we demonstrate that our schemes efficiently and fairly assign the bandwidth to the FL processes for centralized and distributed solutions and outperform a baseline scheme where each edge server assigns bandwidth proportionally to the FL servers' requests that it receives. The proposed distributed and centralized schemes have comptetive performance.

==> eval.tex <==

\section{Evaluations}
\label{sec:eval}
This section presents the empirical evaluation of our proposed game theoretic approach. Each of the  $S$ (e.g., $S=5$), FL Servers is assumed to has $c$ (by default, $c=50$), clients 
that are randomly distributed to $E$ (e.g., $E=5$) edge servers. 
At each round,
each $S_i$ randomly picks $\bar{c}^i{_i} = \lfloor c\cdot\rho \rfloor$ of its clients,
where $\rho$ is a parameter with default value $100\%$. 
Each edge server $E_j$ has a limited number of bandwidth units $b_j$ available;
particularly, $b_j$ should be smaller than the total number of selected clients connected to $E_j$. 

We assumed that each $S_i$ has the same funds for every round. By default, we let $f_i$ be the same for different FL servers could be different when we evaluate the impact of heterogeneity of funds. 

Each $S_i$ is assumed to need $u_i$ units of bandwidth for its clients. By default, we let $u_i=1$ for every FL server, but they
could be different when we evaluate the impact of the required bandwidth unit. 

\subsection{FL baseline scheme}
We assess the effectiveness of the proposed game theoretic approach to resolve the bandwidth allocation problem and compare it to the existing FL baseline scheme where each edge server allocates its available bandwidth to all requesting FL servers proportionally to their requests, applied to widely used datasets and models.  

\subsection{Heterogeneity of client distribution}

To evaluate our proposed scheme with respect to the heterogeneity of client distribution, we used parameters $\alpha$ and $\beta$ to control the heterogeneity of client distribution,
while keeping other parameters the same for all the FL servers and edge servers.

Specifically, when distributing each $S_i$'s $\bar{c}^i$ clients to all the edge servers:
\begin{itemize}
    \item 
    We pick $\alpha\cdot s$ FL servers to distribute their clients only over $\beta\cdot e$ edge servers,
    where $0\leq\alpha\leq1$ and $0\leq\beta\leq1$,
    while the rest $(1-\alpha)\cdot s$ FL servers uniformly randomly distribute their clients to all the $e$ edge servers. 
\end{itemize}
Note that the distribution is uniform when $\alpha=0$ and $\beta=1$.


\subsection{Heterogeneity of funds}

We denote the maximum fund as $1$ and the smallest fund as $f^{0}<1$.  Let $0\leq\gamma\leq 1$, and $\gamma\cdot s$ be the number of FL servers whose funds are between $f^{0}$ and $1$ while the rest (i.e., $(1-\gamma)\cdot s$) FL servers each having the fund of $f^{0}$. More specifically, the $\gamma\cdot s$ FL servers would have funds of $f^{0} + \frac{k\cdot (1-f^{0})}{\gamma\cdot s}$, where $k=1,\cdots, \gamma\cdot s$, respectively, while keeping other parameters same for all the FL servers and edge servers. Under such settings, we will study how the bandwidth allocation is affected by every FL server's funds. 

\subsection{Heterogeneity of required bandwidth units}

Similarly, we now make the value of $u_i$ to be heterogeneous for different FL servers, and different FL servers have different bandwidth requirements and study how it impacts the allocation of bandwidth.

We denote the maximum bandwidth as the number of FL servers, $|S|$,  and the smallest bandwidths as $u_i=1$. 
Let $0\leq\delta\leq 1$, and $\delta\cdot s$ be the number of FL servers whose bandwidths are between $u_i=1$ and $|S|$ while the rest
(i.e., $(1-\delta)\cdot s$) FL servers each having the bandwidths of $u_i$. 
More specifically, the $\delta\cdot s$ FL servers would have bandwidths of $u_i + \frac{k\cdot (|S|-u_i)}{\delta\cdot s}$, where $k=1,\cdots, \delta\cdot s$, respectively. 


